Credible, Truthful, and Two-Round (Optimal) Auctions via Cryptographic Commitments

We consider the sale of a single item to multiple buyers by a revenue-maximizing seller. Recent work of Akbarpour and Li formalizes \emph{credibility} as an auction desideratum, and prove that the only optimal, credible, strategyproof auction is the ascending price auction with reserves (Akbarpour and Li, 2019). In contrast, when buyers' valuations are MHR, we show that the mild additional assumption of a cryptographically secure commitment scheme suffices for a simple \emph{two-round} auction which is optimal, strategyproof, and credible (even when the number of bidders is only known by the auctioneer). We extend our analysis to the case when buyer valuations are $\alpha$-strongly regular for any $\alpha > 0$, up to arbitrary $\varepsilon$ in credibility. Interestingly, we also prove that this construction cannot be extended to regular distributions, nor can the $\varepsilon$ be removed with multiple bidders.

==> archive/archive.tex <==

\begin{lemma}[Extreme Values of MHR distributions (Theorem 19 \cite{cai2011extreme})]\label{lemma:extreme-value-mhr}
Let $X_1, ... , X_n$ be a collection of independent random variables whose distributions are MHR. Then there exists some anchoring point $\beta$
such that $Pr[\sup_i{X_i} \geq \beta/2] \geq 1 - \frac{1}{\sqrt e}$ and
$$ E[\sup_i X_i \cdot \indicator{\sup_i X_i \geq 2 \beta \log 1/\epsilon}] \leq 36\beta \epsilon \log 1/\epsilon \text{, for all $\epsilon \in (0, 1/4)$}$$
\end{lemma}

==> archive/oracle.tex <==

\begin{lemma}\label{lemma:prunning-unsafe-deviation}
Let $S_0$ be a safe deviation, then an auctioneer following strategy $S_0$ always forward all the commitments to all players.
\end{lemma}
\begin{proof}
Let $L_i$ be the list of values committed to player $i$ before the revelation phase. If the value of player $i$ is bigger than all values in the commitment $L_i$, the auctioneer must allocate the item to player $i$ since the auctioneer is unable to proof player $i$ is the winner of the item.

Suppose for contradiction, in strategy $S_0$, the auctioneer is allowed to not forward a commitment for the value of player $i$ to player $j$, $v_i \not \in L_j$. Consider first the case where the auctioneer first observes $v_i$ before observing $v_j$. With half probability $v_i < v_j$, and with non-zero probability $v_i > \max_{v \in L_i} v$ which implies the auctioneer must allocate the item to player $i$. When the auctioneer observes $v_j$, with non-zero probability $v_j > \max_{v \in L_j} v$ which implies the auctioneer must allocate the item to player $j$ which is impossible since the item can only be allocated to a single player.

For the case where the auctioneer first observes $v_j$ before observing $v_i$. With half probability $v_j < v_i$, and with non-zero probability $v_j > \max_{v \in L_j} v$ which implies the auctioneer must allocate the item to player $j$. When the auctioneer observes $v_i$, with non-zero probability $v_i > \max_{v \in L_i} v$ which implies the auctioneer must allocate the item to player $i$. This implies with non-zero probability over player values, strategy $S_0$ is not safe.
\end{proof}

\begin{theorem}\label{thm:mhr}
Assume there is $n$ i.i.d bidders drawn from a MHR distribution $D$. If the entree fee is at least Myerson's optimal reserve on distribution $D$, then the second price auction with commitments is credible.
\end{theorem}
In the proof of Theorem~\ref{thm:mhr}, it is useful to assume a more powerful auctioneer that has access to some advice about bidders private information. We show that not even this powerful auctioneer can profit from deviation let along a weaker one. By considering this powerful auctioneer, we can explicitly compute the optimal strategy and show that it cannot be better as honestly implementing the second price auction with commitments.

\textbf{A simulator.} Given an auctioneer strategy $S_0$ and players $P_1$, ..., $P_n$, we define the simulator $\mathcal S(S_0, P_1^{S_1}, ..., P_n^{S_n})$ as a game where the auctioneer plays game $\mathcal G^{S_0}$ with players $P_1$, ..., $P_n$ where player $i$ follows strategy $S_i$.

\textbf{A mechanism with advice.} Given mechanism $\mathcal M = (\mathcal G, S_n)$, we define the mechanism with advice $\mathcal M^\mathcal O = (\mathcal G^\mathcal O, S_n)$ where the auctioneer can query an oracle $\mathcal O$ that on input $x \in \mathcal X$ outputs function $f : \mathcal X \to \mathbb R$ evaluated on $x$ where $\mathcal X$ is some finite domain.

Next, we will formally define the oracle that allow the auctioneer to learn not only the second highest value among all bidders but also the identity of the highest value bidder.

\textbf{A second price oracle} Let $i^*$ be the index of the player of highest value breaking ties in favor of lower indexes. For each player $i$, define $f(i) = v_i$ if $i \neq i^*$ and $f(i) = \bot$ if $i = i^*$ where $\bot$ represents fail. Define the second price oracle $\mathcal O$ as the oracle that when queried on input $i$ outputs $f(i)$.

By giving the auctioneer oracle access to the second price oracle $\mathcal O$, after querying the oracle on inputs $1$ to $n$, the auctioneer learns that player $i^*$ has the highest value and that the second highest value is $v_j$, $j \neq i^*$. It follows, $v_{i^*}$ is distributed according to $F_{X| X \geq v_j}(x) = Pr_{v_{i^*} \leftarrow D}[v_{i^*} \leq x | v_{i^*} \geq v_j]$.

Clearly, $\Rev(\mathcal M^\mathcal O, S_n) \geq \Rev(\mathcal M, S_n)$ because for all strategy $S_0$ of the auctioneer implementing game $\mathcal G$, the auctioneer can follow the same strategy on game $\mathcal G^\mathcal O$ without doing any oracle queries and get the same revenue on expectation. Next, we formalize the idea of the auctioneer running auctions in parallel.

\textbf{A parallel game.} A $k$-parallel game is a collection of $k$ games $(\mathcal S(S_0^i, P^i))_{i = 1}^k$ where $S_0^i$ is the auctioneer's strategy on game $i$, and $P^1, ..., P^k$ is a partition of the players. For each player $i \in N$, we specify a strategy $S_i$ for player $i$ in the game. Each parallel game pauses before the start of the allocation phase, and the auctioneer allocates the item to the game that gives higher revenue. 

In Lemma~\ref{lemma:prunning-strategies}, when the auctioneer has access to the second price oracle, we show it is without loss to consider only 2-parallel games.

\begin{lemma}\label{lemma:prunning-strategies}
Assume $\mathcal O$ is the second price oracle. If $S_0^\mathcal O$ is a safe deviation on SPC, there is a safe deviation $S_0^\mathcal O'$ where:
\begin{itemize}
    \item The auctioneer plays strategy $S^{SPC}$ with player $P_2, ..., P_n$ and don't allocate the item.
    \item The auctioneer only allocate the item to player 1.
    \item $E[u_0(S_0^\mathcal O', S_N, v)] \geq E[u_0(S_0^\mathcal O, S_N, v)]$.
\end{itemize}
\end{lemma}
\begin{proof}
Define $S_0^\mathcal O'$ as follows. Before the game starts, the auctioneer queries the oracle and learns the identity of the highest value player and the second highest value. Without loss of generality, let $v_1 \geq v_2 \geq ... \geq v_n$ be order of values where the only unknown for the auctioneer is $v_1$.

The auctioneer first simulate an SPC auction with players $2, ..., 3$ and don't allocate the item in the allocation phase. Next, the auctioneer simulate another SPC auction $\mathcal A$ only with player 1.

Let $rev = E_{v_1 \leftarrow D_1}[u_0(S_0^\mathcal O, S_N, v)| v_2, ..., v_n]$ be the auctioneer's expected revenue on strategy $S_0^\mathcal O$ after the auctioneer learns $v_2, ..., v_n$. In auction $\mathcal A$, if $rev \leq v_2$, in the commitment phase, the auctioneer only commits to $v_2$. In the allocation phase, the auctioneer allocates the item to player 1 which pays $v_2$. This implies,

\begin{align*}
    E_{v_1 \leftarrow D_1}[u_0(S_{0}^{\mathcal O'}, S_N, v) \cdot \indicator{rev \leq v_2}| v_2, ..., v_n] &= v_2 \geq E_{v_1 \leftarrow D_1}[u_0(S_0^{\mathcal O}, S_N, v)| v_2, ..., v_n]
\end{align*}

If $rev > v_2$, the auctioneer simulates $S_0^\mathcal O$ with player 1 and dummy players for players $2, ..., n$. Dummy player $i$, plays strategy $S_i^{SPC}$ with value $v_i$. In the end of the simulation, the auctioneer only gets a payment if the item is allocated to player 1. This implies,

\begin{align*}
    E_{v_1 \leftarrow D_1}[u_0(S_0^{\mathcal O'}, S_N, v) \cdot \indicator{rev > v_2}| v_2, ..., v_n] &= 
\end{align*}

\begin{align*}
    E_{v \leftarrow D}[u_0(S_0^\mathcal O', S_N, v)] &= E_{v_{-1} \leftarrow D_{-1}}[E_{v_1 \leftarrow D_1}[u_0(S_0^\mathcal O', S_N, v)| v_2, ..., v_n]]\\
    &= 
\end{align*}
\end{proof}

\begin{lemma}
Assume $\mathcal G$ is the game described by the second price auction with commitments (SPC), and $\mathcal O$ is the second price oracle. If $S_0$ is a safe deviation for the auctioneer on game $\mathcal G$, there is a safe deviation $S_0'$ where $S_0'$ is a 2-parallel game:
\begin{itemize}
    \item In the first game, player 1 plays against $n-1$ dummy players, $\mathcal E_1 = \mathcal S(S_0^{(1)}, P_1, \tilde P_2, ..., \tilde P_n)$.
    \item In the second game, players $2, ..., n$ play against one dummy player, $\mathcal E_2 = \mathcal S(S_0^{(2)}, \tilde P_1, P_2, ..., P_n)$.
    \item Dummy player $\tilde P_i$, $i \neq 1$, follows strategy $S^{SPC}(v_i)$.
    \item Dummy player $\tilde P_1$, relay messages from player $P_1$ on game $\mathcal E_1$.
    \item Strategies $S_0^{(1)}$ and $S_0^{(2)}$ are a safe deviation from $S_0^{\mathcal G}$.
    \item $S_0'$ gives at least the same revenue:
    $$E_{v \leftarrow D}[u_0(S_0', S_N, v)] = E_{v \leftarrow D}[u_0(S_0, S_N, v)]$$ 
\end{itemize}
\end{lemma}
\begin{proof}
Strategy $S_0'$ proceeds as follows.  The auctioneer is going to going run two parallel games.

In the first game, the auctioneer simulates a game following strategy $S_0^{(1)}$ with only player 1 and simulating $n-1$ dummy players $\tilde P_2, ..., \tilde P_n$. Let $\mathcal E_1 = \exec(S_0^{(1)}, P_1, \tilde P_2, ..., \tilde P_n)$ denote such execution. Strategy $S_0^{(1)}$ is identical to $S_0$ except that the simulation proceeds as follows:
\begin{itemize}
    \item When the auctioneer is called to activate player $i$, the auctioneer activates dummy player $\tilde P_i$ instead.
    \item When a dummy player is active, they behave as a true player following strategy $S_i^\mathcal G$ with value $v_i$.
\end{itemize}
In the second game, the auctioneer simulates a game following strategy $S_0^{(2)}$ with all players except player 1. Player 1 is replaced by a dummy player $\tilde P_1$. Let $\mathcal E_2 = \exec(S_0^{(2)}, \tilde P_1, P_2, ..., P_n)$ denote such execution. Strategy $S_0^{(2)}$ is identical to $S_0$ except that the simulation proceeds as follows:
\begin{itemize}
    \item When the auctioneer is called to activate player 1, the auctioneer activates dummy player $\tilde P_1$ instead.
    \item When $\tilde P_1$ is active, the auctioneer waits for true player $P_1$ to answer the same query on game $\mathcal E_1$. $\tilde P_1$ replies what $P_1$ replies. The only time $\tilde P_1$ is active is when the auctioneer request a commitment, and when the auctioneer request the commitment to be opened. Because $S_0^{(1)}$ is a safe deviation from $S_0^\mathcal G$, the auctioneer always activates player 1 to request a commitment and request the commitment to be open. 
\end{itemize}

The outcome of game $\mathcal E_1$ and $\mathcal E_2$ are the same with the only exception that if the item is allocated to $\tilde P_i$ in $\mathcal E_1$, the item is allocated to $P_i$ in $\mathcal E_2$. If the item is allocated to $P_1$ in $\mathcal E_1$, the item is allocated to $\tilde P_1$ in $\mathcal E_2$.  The auctioneer ignores the allocation to the dummy player and allocates to the real player. In the allocation phase, $S_0^{(1)}$ and $S_0^{(2)}$ behave like $S_0$; therefore, $E_{v \leftarrow D}[u_0(S_0', S_N, v)] = E_{v \leftarrow D}[u_0(S_0, S_N, v)]$.
\end{proof}

\begin{lemma}\label{lemma:cond-optimal-reserve}
Assume there is a single bidder with value $v$ distributed according to a regular distribution $D$. Assume $v_1 \geq v_2$, then the optimal truthful auction is a posted price auction with price:
$$p = \max\{v_2, \phi_F^{-1}(0)\} = \arg \max_p p Pr_{v_1 \leftarrow D}[v_1 \geq p | v_1 \geq v_2]$$
\end{lemma}
\begin{proof}
By Myerson's Lemma and fact $D$ is regular, the optimal revenue is obtained when we maximize the virtual welfare $\max_\pi E[\pi(v_1)\phi_{F_{X|X \geq v_2}}(v_1)]$ where $\pi(v_1) = 1$ iff we sell the item (otherwise $\pi(v_1) = 0$). We have:
\begin{align*}
    F_{X|X \geq v_2}(x) = Pr[v_1 \leq x | v_1 \geq v_2] &= 1 - Pr[v_1 > x | v_1 \geq v_2]\\
    &= 1 - \frac{Pr[v_1 > x, v_1 \geq v_2]}{Pr[v_1 \geq v_2]}\\
    &= 1 - \frac{1 - F(\max(x, v_2))}{1 - F(v_2)}
\end{align*}
The density function is given by,
\begin{align*}
    Pr[v_1 = x | v_1 \geq v_2] = \begin{cases}
    0 & \text{, if $x < v_2$}\\
    \frac{f(x)}{1 - F(v_2)} & \text{, if $x \geq v_2$}
    \end{cases}
\end{align*}
It follows,
\begin{align*}
    &E_{v_1 \leftarrow F_{X|X\geq v_2}}[\pi(v_1)\phi_{F_{X|X \geq v_2}}(v_1)]\\
    &\quad= E_{v_1 \leftarrow F_{X|X\geq v_2}}\bigg[\pi(v_1)
    \bigg(v_1 - \frac{1 - F(\max(v_1, v_2))}{1-F(v_2)}\frac{1 - F(v_2)}{f(v_1)}\bigg) \bigg]\\
    &\quad=E_{v_1 \leftarrow F_{X|X\geq v_2}}\bigg[\pi(v_1)\bigg(v_1 - \frac{1 - F(v_1)}{f(v_1)}\bigg) \bigg]\\
    &\quad=E_{v_1 \leftarrow F_{X|X\geq v_2}}[\pi(v_1)\phi_F(v_1)]
\end{align*}
Let $r = \inf\{x | Pr[v_1 = x | v_1 \geq v_2] > 0, \phi_F(v) \geq 0\}$, then the virtual welfare is maximized when $\pi(v) = 0$ for all $v < r$ and $\pi(v) = 1$ for all $v \geq r$. We conclude $p = \phi^{-1}_F(0)$ when $\phi^{-1}_F(0) \geq v_2$ and $p = v_2$ when $\phi^{-1}_F(0) < v_2$ which concludes the proof.
\end{proof}

\begin{lemma}\label{lemma:mhr-opt-single-bidder}
Assume $D$ is MHR with cumulative density function $F$. Assume there is a single bidder with value $v_1$ drawn from $D_{X | X \geq v_2}$ for some $v_2 \in \mathbb R^+$. Let $r = \phi_F^{-1}(0)$ be Myerson's reserve. If the entree fee $k \geq r$, the maximum revenue of all safe deviations for the auctioneer in the second price auction with commitments is $\max\{v_2, r Pr[v_1 \geq r | v_1 \geq v_2]\}$.
\end{lemma}
\begin{proof}
In the SPC, the auctioneer must announce the number of bidders as $n = 1$ and post the optimal reserve price for the distribution $D_{X | X \geq v_2}$ which from Lemma~\ref{lemma:cond-optimal-reserve} is $\max\{v_2, \phi_F^{-1}(0)\}$. Suppose instead the auctioneer announces $n = 1 + m$ players with the intent of submitting $m$ fake bids. In the commitment phase, the auctioneer commits to bids $x_1 > x_2 > ... > x_m$. Without loss of generality, $x_1 \geq v_2$ since the auctioneer is guaranteed to always get a payment of $v_2$ by committing on $v_2$.

In the revelation phase, the auctioneer observes $v_1$ and in the allocation phase, the auctioneer can decide which commitments to open for the bidder to maximize payments. Without loss of generality, assume $x_i \geq k(m-i)$; otherwise, the auctioneer never gets payment from committing to $x_i$. To get the bidder to pay $x_i$, it must hide bids $x_{i+1}, ..., x_m$ which requires the auctioneer to pay $k(m - i)$ as penalty.

Consider the case where $v_1 \in [x_i, x_{i+1})$. Without loss of generality, the auctioneer reveals $x_1, ..., x_i$ and hides $x_{i+1}, ..., x_{m}$ paying $k(m - i)$ as penalty. Assume the contrary. If the auctioneer reveals any value above or equal to $x_{i+1}$, the auctioneer cannot declare $v_1 < x_{i+1}$ as the winner; therefore, it gets no payment. If the auctioneer, hides any value smaller or equal than $x_i$, the auctioneer can only decrease the payment of the bidder in exchange for paying higher penalties.

Let $S_0$ denotes the auctioneer's revenue maximizing strategy, and let $S_1$ denotes the bidder strategy when playing on the SPC. By the previous argument, we have the following expression for the expected revenue,

\begin{observation}\label{obs:opt-revenue}
If the auctioneer commits to $m$ fake bids $\max\{v_2, k(m-1)\} \leq x_1 \leq ... \leq x_n$, the optimal auctioneer's revenue is:
\begin{align*}
    E_{v_1 \leftarrow F_{X | X \geq v_2}}[u_0(S_0, S_1, v_1)] &= \sum_{i = 1}^m(x_i - k(m-i))Pr[v_1 \in [x_i, x_{i+1}) | v_1 \geq v_2]\\
    &\quad + \max\{0, v_2 - km\}Pr[v_1 < x_1 | v_1 \geq v_2]
\end{align*}
where we define $x_{m+1} = \inf\{x | F(x) = 1\}$.
\end{observation}

Let's first consider the case where $v_2 \leq km$. We will show that the expected revenue is at most $x_1 Pr_{v_1 \leftarrow F_{X | X \geq v_2}}[v_1 \geq x_1]$ which is the expression for the revenue on a posted price auction with posted price $x_1$ on distribution $D_{X | X \geq v_2}$ which by Lemma~\ref{lemma:cond-optimal-reserve} is $\max\{v_2, r Pr[v_1 \geq r | v_1 \geq v_2]\}$.

If $m = 1$, it is easy to see from Observation~\ref{obs:opt-revenue} that
\begin{align*}
E_{v_1 \leftarrow F_{X | X \geq v_2}}[u_0(S_0, S_1, v_1)] &= x_1 Pr_{v_1 \leftarrow F_{X | X \geq v_2}}[v_1 \geq x_1]\\
&\leq \max\{v_2, r Pr[v_1 \geq r | v_1 \geq v_2]\} \text{, by Lemma~\ref{lemma:cond-optimal-reserve}}
\end{align*}

If $m \geq 2$, by rearranging the auctioneer's revenue (Observation~\ref{obs:opt-revenue}):

\begin{align*}
    &E_{v_1 \leftarrow F_{X | X \geq v_2}}[u_0(S_0, S_1, v_1)] = \sum_{i = 1}^m(x_i - k(m-i))Pr[v_1 \in [x_i, x_{i+1}) | v_1 \geq v_2]\\
    &= \sum_{i = 1}^m(x_i - k(m-i))\frac{F(x_{i+1}) - F(x_i)}{1 - F(v_2)}\\
    &= \sum_{i = 1}^m x_i \frac{1 - F(x_i)}{1 - F(v_2)} - 
    \sum_{i = 1}^{m-1} \frac{k(m - i)(F(x_{i+1}) - F(x_i)) + x_i(1 - F(x_{i+1}))}{1 - F(v_2)}\\
\end{align*}
We first claim that $(F(x_{i+1}) - F(x_i)) \geq \frac{(1 - F(x_{i+1}))(x_{i+1} - x_i)}{k}$. For that, observe that if a distribution is regular and $x \geq \phi^{-1}(0)$, then we can lower bound the hazard rate $h(x) = \frac{f(x)}{1 - F(x)} \geq \frac{1}{x}$.
\begin{lemma}\label{lemma:regular-bound}
Assume $F$ is regular. If $x \geq \phi^{-1}(0)$, then $h(x) \geq \frac{1}{x}$
\end{lemma}
\begin{proof}
If $F$ is regular, $\phi(x)$ is monotone increasing and $\phi(x) \geq 0$. We have $\phi(x) = x - \frac{1 - F(x)}{f(x)}$ then $h(x) = \frac{f(x)}{1 - F(x)} \geq x$.
\end{proof}

Bellow, in the first inequality, we use the fact $x_i \geq k(m-1) \geq k \geq \phi^{-1}(0)$ since $m \geq 2$.
\begin{align*}
    F(x_{i+1}) - F(x_i) &= \int_{x_i}^{x_{i+1}} f(x) dx &\\
    &= \int_{x_i}^{x_{i+1}} f(x)\frac{1 - F(x)}{1- F(x)} dx\\
    &\geq \frac{f(k)}{1 - F(k)}\int_{x_i}^{x_{i+1}} 1 - F(x) dx  \quad \text{($F$ is MHR and $x_i \geq k$)}\\
    &\geq \frac{f(k)}{1 - F(k)}(1 - F(x_{i+1}))(x_{i+1} - x_i) \quad \text{($1-F(x)$ is monotone decreasing)}\\
    &\geq \frac{(1- F(x_{i+1})(x_{i+1} - x_i)}{k} \quad\text{($x_i \geq k$ and by Observation~\ref{lemma:regular-bound})}
\end{align*}

Plugging it back in the auctioneer's revenue,
\begin{align*}
&E_{v_1 \leftarrow F_{X | X \geq v_2}}[u_0(S_0, S_1, v_1)]\\
&\quad= \sum_{i = 1}^m x_i \frac{1 - F(x_i)}{1 - F(v_2)} - 
    \sum_{i = 1}^{m-1} \frac{k(m - i)(F(x_{i+1}) - F(x_i)) + x_i(1 - F(x_{i+1}))}{1 - F(v_2)}\\
&\quad\leq \sum_{i = 1}^m x_i \frac{1 - F(x_i)}{1 - F(v_2)} - \sum_{i = 1}^{m - 1} \frac{k\frac{(1 - F(x_{i+1}))(x_{i+1} - x_i)}{k} + x_i(1 - F(x_{i+1}))}{1 - F(v_2)}\\
&\quad= \sum_{i = 1}^m x_i \frac{1 - F(x_i)}{1 - F(v_2)} - \sum_{i = 1}^{m - 1} \frac{(1 - F(x_{i+1}))(x_{i+1} - x_i + x_i)}{1 - F(v_2)}\\
&\quad= \sum_{i = 1}^m x_i \frac{1 - F(x_i)}{1 - F(v_2)} - \sum_{i = 2}^{m} \frac{x_i(1 - F(x_{i}))}{1 - F(v_2)}\\
&\quad= x_1 \frac{1 - F(x_1)}{1 - F(v_2)}\\
&\quad= x_1 Pr[v_1 \geq x_1 | v_1 \geq v_2]\\
&\quad\leq \max\{v_2, r Pr[v_1 \geq r | v_1 \geq v_2]\} \quad \text{(by Lemma~\ref{lemma:cond-optimal-reserve})}
\end{align*}

Let's now consider the case where $v_2 > km$. We have $v_2 \geq r$ which by Lemma~\ref{lemma:cond-optimal-reserve} implies the optimal price for a posted price auction with value distribution $D_{X | X \geq v_2}$ would be to post price $v_2$ and sell with probability 1.  Let $x_i = v_2 + \Delta_i$ for $\Delta_i > 0$. Define $x_0 = v_2$ and $\Delta_0 = 0$, then
\begin{align*}
&E_{v_1 \leftarrow F_{X | X \geq v_2}}[u_0(S_0, S_1, v_1)] = \sum_{i = 1}^m(x_i - k(m-i))Pr[v_1 \in [x_i, x_{i+1}) | v_1 \geq v_2]\\
&\quad + (v_2 - km)Pr[v_1 < x_1 | v_1 \geq v_2]\\
&= v_2\sum_{i = 0}^m \frac{F(x_{i+1}) - F(x_{i})}{1 - F(v_2)} + \sum_{i = 0}^m (\Delta_i - k(m-i))\frac{F(x_{i+1}) - F(x_i)}{1 - F(v_2)}\\
&= v_2 + \frac{Gain(\Delta)}{1 - F(v_2)}
\end{align*}
where $Gain(\Delta) = \sum_{i = 0}^m (\Delta_i - k(m-i))(F(x_{i+1}) - F(x_i))$. In the limit, as $\Delta_i \to 0$ for all $i$, $Gain(\Delta) \to 0$ and the revenue is the same as the revenue of the optimal honest auction. Next, we show that all the partial derivatives $\frac{d}{d \Delta_i}$ of $Gain(\Delta)$ are at most 0 which implies that $\Delta_i = 0$ for all $i$ maximizes the auctioneer's revenue.

\begin{claim}
For all $i \in [m]$, $\frac{d Gain(\Delta) }{d \Delta_i} \leq 0$
\end{claim}
\begin{proof}
\begin{align*}
    & \frac{d Gain(\Delta) }{d \Delta_i} = F(x_{i+1}) - F(x_i) - (\Delta_i - k(m-1))f(x_i)\\
    &\quad + (\Delta_{i-1} - k(m-i+1))f(x_i)\\
    &\quad \leq 1 - F(x_i) - f(x_i)(\Delta_i - \Delta_{i-1} + k) \quad \text{(since $F(x_{i+1}) \leq 1$)}\\
    &\quad= (1 - F(x_i))\bigg(1 - (\Delta_i - \Delta_{i-1} + k)\frac{f(x_i)}{1 - F(x_i)}\bigg)\\
    &\quad\leq (1 - F(x_i))\bigg(1 - \frac{(\Delta_i - \Delta_{i-1} + k)}{k}\bigg)\\
    &\quad\text{(since $x_i \geq v_2 \geq k$, the MHR property and Observation~\ref{lemma:regular-bound})}\\
    &\quad\leq 0 \text{(since $\Delta_{i-1} \leq \Delta_{i}$)}
\end{align*}
\end{proof}
This concludes the proof and the auctioneer can get revenue at most $\max\{v_2, r Pr[v_1 \geq r | v_1 \geq v_2]\}$.
\end{proof}

\begin{corollary}\label{cor:opt-revenue}
Let $\mathcal G^\mathcal O$ be the game described by the second price auction with commitments with access to the second price oracle. Let $r$ be Myerson's reserve and let $D$ be a MHR distribution. The optimal revenue for the auctioneer over all safe deviations when $k \geq r$ is $\max\{v_2, r Pr_{v_1 \leftarrow D}[v_1 \geq r | v_1 \geq v_2]\}$.
\end{corollary}
\begin{proof}
By Lemma~\ref{lemma:prunning-strategies}, when maximizing revenue, is without loss of generality to consider the parallel execution of the following games:
$$\mathcal E_1 = \mathcal S(S_0^{(1)}, P_1, \tilde P_2, ..., \tilde P_n)$$
$$\mathcal E_2 = \mathcal S(S_0^{(2)}, \tilde P_1, P_2, ..., P_n)$$
where the complete description of the game can be found in the proof of Lemma~\ref{lemma:prunning-strategies}. In each run of the parallel game, the item can be allocated to only one of the games which implies we can bound the revenue of the parallel game as the maximum revenue of the individual games. $S_0^{(1)}$ is a safe deviation from SPC and the game implemented by $S_0^{(1)}$ is an auction with a single bidder supported on distribution $D_{X | X \geq v_2}$. By Lemma~\ref{lemma:mhr-opt-single-bidder}, such game can give revenue at most $\max\{v_2, r Pr_{v_1 \leftarrow D}[v_1 \geq r | v_1 \geq v_2]\}$. The second game gives revenue at most $v_2$ since all players have value at most $v_2$. Combining the upper bounds for the revenue of $\mathcal E_1$ and $\mathcal E_2$, we have that the parallel game has revenue at most $\max\{v_2, r Pr_{v_1 \leftarrow D}[v_1 \geq r | v_1 \geq v_2]\}$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:mhr}]
Let $S_0^\mathcal O$ be the optimal auctioneer strategy in game $\mathcal G^\mathcal O$ where $\mathcal O$ is the second price oracle. Because $S_0^\mathcal O$ is optimal, we have
\begin{align*}
    E[u_0(S_0^{SPC}, S_N, v)] \leq E[u_0(S_0^\mathcal O), S_N, v)]
\end{align*}
By Corollary~\ref{cor:opt-revenue}, $S_0^\mathcal O$ gets revenue at most $\max_i^{(2)} v_i$ when $\max_i^{(2)} v_i \geq r$

\begin{align*}
&E[u_0(S_0^{SPC}, S_N, v)] = E[u_0(S_0^{SPC}_0, S_N, v) \cdot \indicator{\max^{(2)}_i v_i \geq r}]\\
&\quad\quad+ E[u_0(S_0^{SPC}, S_N, v) \cdot \indicator{\max^{(2)}_i v_i < r}]\\
&\quad= E[\max^{(2)}_i v_i | \max^{(2)}_i v_i \geq r]Pr[\max^{(2)}_i v_i \geq r]\\
&\quad\quad+ r Pr[\max^{(1)}_i v_i \geq r | \max^{(2)}_i v_i < r]Pr[\max^{(2)}_i v_i < r]\\
&\quad = E[u_0(S_0^\mathcal O, S_N, v)]
\end{align*}
\end{proof}

==> archive/second-price-commitment-auction.tex <==
In setup phase, the auctioneer announces the number $n$ of bidders and a commitment fee $k$. Initialize $A = \emptyset$. The game proceeds as follows:

\textbf{Commitment Phase}
\begin{itemize}
    \item For all $i \in [n]$, the auctioneer activates bidder $i$ and request bidder $i$ to reply with a commitment for their bid. When bidder $i$ is active:
    \begin{itemize}
        \item Bidder $i$ draws a uniformly-random string $r_i \leftarrow \{0, 1\}^\lambda$.
        \item Bidder $i$ replies $c_i = \commit(v_i, r_i)$ and deposit the commitment fee $k$.
    \end{itemize}
    \item Update $n$ if a bidder aborted before sending their bid.
    \item For all $i \in [n]$, the auctioneer sends $c_{-i}$ to bidder $i$.
\end{itemize}

\textbf{Revelation Phase}
\begin{itemize}
    \item For all $i \in [n]$, the auctioneer activates bidder $i$ and request bidder $i$ to open commitment $c_i$. When bidder $i$ is active:
    \begin{itemize}
        \item Bidder $i$ replies $(v_i', r_i')$.
        \item The auctioneer checks $c_i \overset{?}{=} \commit(v_i', r_i')$. If $c_i = \commit(v_i, r_i)$, update $A = A \cup \{i\}$ and returns the commitment fee to bidder $i$; otherwise, the auctioneer aborts bidder $i$.
    \end{itemize}
\end{itemize}

\textbf{Allocation Phase}
\begin{itemize}
    \item The auctioneer allocates the item to bidder $i^* = \arg \max_{i \in A} v_i$ and charges price $p_{i^*} = \max_{i \in A/\{i^*\}}$, $p_{-i^*} = 0$.
\end{itemize}

\textbf{Verification Phase}
\begin{itemize}
    \item \textbf{Proof of payment.} The auctioneer opens the commitments $c_{-i^*}$ to bidder $i^*$ by sending $\{(v_i, r_i)\}_{i \in A/\{i^*\}}$.
    \item \textbf{Proof of allocation.} The auctioneer opens commitment $c_{i^*}$ to bidder $j \neq i^*$ by sending $(v_{i^*}, r_{i^*})$.
    \item \textbf{Payment of penalties.} The auctioneer gives bidder $i^*$ the commitment fee of bidders that aborted.
\end{itemize}

\subsection{Remarks about the bidding space} For the analysis, we will assume bidders drawn uniformly-random quantile $q = [0, 1]$ and the highest bid is the bid with highest quantile. In this setting, the probability of a draw between bidders is zero. Given access to the distribution $D$, a bid can be converted to the value space by computing the inverse $v = F^{-1}(q)$. Note that $v$ is identically distributed to $D$:
\begin{align*}
    Pr[v \leq x] &= Pr[F(v) \leq F(x)]\\
    &= Pr[q \leq F(x)]\\
    &= F(x)\quad\text{(Because $q$ is drawn uniformly-random from $[0, 1]$)}
\end{align*}

In this paper, we will assume bidders can communicate and compute commitments to quantiles. In practice, bidders can only communicate a finite number of bits; however, the bidding space can easily be made finite through a discretization of the quantile space as $Q = \{0, 1/N, ..., (N-1)/N\}$ for some power of two $N \in \mathbb Z^+$.



==> archive/second-price.tex <==
\begin{theorem}\label{thm:strongly-regular-bound}
Assume the commitment fee $k$ is at least the optimal reserve price $r$. If bidders are i.i.d from an $\alpha$-strongly regular distribution $D$, then the auctioneer's revenue is at most
$$E_{v \leftarrow D}[\max_{i \in [n]}\phi^+(v_i)] + \frac{1-\alpha}{\alpha}E_{v \leftarrow D}[\max_{j \in [n]}\phi(v_i) \cdot \indicator{\exists i \in [n], v_i \geq k}]$$
\end{theorem}
\begin{proof}
Let $s_0$ be the auctioneer's strategy that implements the second-price auction with commitments and let $s_0'$ be the optimal safe deviation from $s_0$. Let $s = (s_1, s_2, ..., s_n)$ be the strategy profile of all bidders specified by the second-price auction with commitments.

During the execution of $s_0'$, let $b_i \subseteq v$ be the subset of bids observed by the auctioneer before forwarding commitments to bidder $i$. Let $x^i(b_i) = (x_1^i, ..., x_{m_i(b_i)}^i)$ be the state of commitments forwarded to bidder $i$. Without loss of generality, let $x^i_1 < x^i_2 < ... < x^i_{m_i(b_i)}(v)$. Note that $x^i(b_i)$ is a random vector where the dimension $m_i(b_i)$ is a random variable depending on the transcript observed so far. After observing all bids $v = (v_1, v_2, ..., v_n)$, $x^i(v)$ is completely determined for all $i \in [n]$. Also observe $x^i(v) = x^i(v_{-i})$ since before sending $x^i(v)$, the auctioneer only observes $Commit(v_i, r_i)$ which reveals nothing about $v_i$ since the commitment is perfectly hiding.

The next claim bounds the revenue for the case where there is a bidder $i \in [n]$ where $v_i > x^i_{m_i(v)}(v)$:
\begin{claim}\label{claim:large-values}
For every safe deviation $S$,
$$E[u_0(s_0', s, v) \cdot \indicator{\exists i \in [n], v_i > x_{m_i(v)}^i(v)}] \leq E[\max_{j \in [n]} \phi^+(v_j) \cdot \indicator{\exists i \in [n], v_i > x^i_{m_i(v)}(v)}]$$
\end{claim}
\begin{proof}
If $v_i > x^i_{m_i(v)}(v)$, the item must be allocated to bidder $i$ since there is no commitments the auctioneer can open to bidder $i$ to proof that bidder $i$ is not the winner. This implies for all $j \neq i$, events $\{v_i > x^i_{m_i(v)}\}$ and $\{v_j > x^j_{m_j(v)}\}$ are disjoint; otherwise, strategy $s_0'$ is not safe and risks having to allocate the same item to two distinct bidders. In addition, if $v_i > x^i_{m_i(v)}(v)$, the auctioneer must open all commitments and allocate the item to bidder $i$ and get $x^i_{m_i(v)}(v)$ as payment.

\begin{align*}
E_{v \leftarrow D}&[u_0(s_0', s, v) \cdot \indicator{\exists i \in [n], v_i > x_{m_i(v)}^i(v)}]\\
&= \sum_{i = 1}^n E_{v \leftarrow D}[u_0(s_0', s, v) \cdot \indicator{v_i > x^i_{m_i(v)}(v)}]\\
&= \sum_{i = 1}^n E_{v \leftarrow D}[x^i_{m_i(v)}(v) \cdot \indicator{v_i > x^i_{m_i(v)}(v)}]
\end{align*}

There is a truthful mechanism that gets the same allocation and payment:
\begin{itemize}
    \item Request a bid from all bidders.
    \item Compute $x^i_{m_i(v_{-i})}(v_{-i})$ for all $i \in [n]$ and give the item to bidder $i$ at price $x^i_{m_i(v_{-i})}(v_{-i})$ if $v_i > x^i_{m_i(v_{-i})}(v_{-i})$. If $v_i \leq x^i_{m_i(v_{-i})}(v_{-i})$ for all $i \in [n]$, don't allocate the item.
\end{itemize}
The mechanism computes a valid allocation -- if $x$ was generated by the transcript of a safe deviation, the item can only be allocated to a single bidder. It is easy to see the mechanism is Dominant-Strategy Incentive-Compatible (DSIC). For a bidder $i$ that wins the item, that bidders deviation to $v_i' \neq v_i$ cannot change the allocation or the payment $x^i_{m_i(v_{-i})}(v_{-i})$. For a bidder $i$ that does not win the item, any deviation cannot change the allocation. By Myerson's theorem, the revenue of our truthful mechanism is
\begin{align*}
    \sum_{i = 1}^n E[x^i_{m_i(v_{-i})}(v_{-i}) \cdot \indicator{v_i > x^i_{m_i(v_{-i})}(v_{-i})}] = \sum_{i = 1}^n E[\phi(v_i) \cdot \indicator{v_i > x^i_{m_i(v_{-i})}(v_{-i})}]
\end{align*}
Because $\phi(\cdot)$ is regular, $\phi(\cdot)$ is monotone increasing, then
\begin{align*}
    E[\phi(v_i) \cdot \indicator{v_i > x^i_{m_i(v_{-i})}(v_{-i})}] \leq E[\max_{j \in [n]} \phi^+ (v_j) \cdot \indicator{v_i > x^i_{m_i(v_{-i})}(v_{-i})}]
\end{align*}
Putting it all together,
\begin{align*}
    \sum_{i = 1}^n E[&u_0(s_0', s, v) \cdot \indicator{v_i > x^i_{m_i(v)}(v)}] \leq \sum_{i = 1}^n E[\max_{j \in [n]}\phi^+(v_j) \cdot \indicator{v_i > x_{m_i(v)}^i(v)}]\\
    &= E_{v \leftarrow D}[\max_{j \in [n]}\phi^+(v_j) \cdot \indicator{\exists i \in [n], v_i > x^i_{m_i(v_{-i})}(v_{-i})}]
\end{align*}
where the last equality follows by the fact the events in the indicator are disjoint.
\end{proof}

The next claim bounds the revenue for the case where for all bidders $i \in [n]$, $v_i < x_{m_i(v_{-i})}^i(v_{-i})$.

\begin{claim}\label{claim:small-values}
For all safe deviations $S$,
$$E[u_0(s_0', s, v) \cdot \indicator{\forall i \in [n], v_i < x^i_{m_i(v)}(v)}] \leq E[\max_{j \in [n]}\phi^+(v_j)\cdot \indicator{\forall i \in [n], v_i < x^i_{m_i(v)}(v)}]$$
\end{claim}
\begin{proof}
For all bidders $i \in [n]$, even though $v_i < x^i_{m_i(v_{-i})}(v_{-i})$, the auctioneer can allocate the item to bidder $i$ by revealing all $x^i_\ell(v)$ if $x^i_\ell < v_i$ and hiding $x_\ell^i(v)$ if $x^i_\ell(v) > v_i$. For bidder $j \neq i$, the auctioneer reveals everything proving to bidder $j$ that they are not the winner. Let $p_i(v)$ be the profit the auctioneer can obtain by allocating the item to bidder $i$ which is a random variable depending on $v$. We must have $p_i(v) \leq v_i - k$ since the payment can be at most $v_i$ and the penalties are at least $k$ since the auctioneer must hide at least one bid from bidder $i$. We might have $p_i(v) < 0$ if the penalties are higher than $v_i$ in which case is in the auctioneer's best interest to not allocate the item to bidder $i$.

Let $A$ denote the set of bidders with non-negative profit, $A = \{i | p_i(v) \geq 0\}$. The optimal strategy for the auctioneer is to allocate the item to the bidder that gives the highest non-negative profit and not allocate if $A = \emptyset$ which implies
\begin{align*}
    u_0(s_0', s, v) &= \max_{i \in A} p_i(v)\\
    &\leq \max_{i \in A} v_i - k
\end{align*}
If the revenue is non-zero, we must have $v_i > k$ for some $i \in [n]$. Because $k \geq r$ and $p_i(v) \geq 0$, we must have $v_i \geq k$ which allow us to invoke Lemma~\ref{lemma:alpha-penalty}:
\begin{align*}
    E[&u_0(s_0', s, v) \cdot \indicator{\forall i \in [n], v_i < x^i_{m_i(v)}(v)}]\\
    &\leq E_{v \leftarrow D}[\max_{j \in A} v_j(v) - k \cdot \indicator{\forall i\in [n] \in [n], v_i < x^i_{m_i(v)}(v)}]\\
    &\leq E_{v \leftarrow D}[\phi(\max_{i \in A} v_i)\cdot \indicator{\forall i\in [n], v_i < x^i_{m_i(v)}(v)}] \\
    &\quad+ \frac{(1-\alpha)}{\alpha}E[\phi(\max_{i \in A} v_i) \indicator{\forall i\in [n], v_i < x^i_{m_i(v)}(v)}]\quad \text{(By Lemma~\ref{lemma:alpha-penalty})}
\end{align*}
The statement follows by observing the distribution is regular which implies the virtual value function is monotone increasing.
\end{proof}

Claim~\ref{claim:large-values} and Claim~\ref{claim:small-values} together implies the theorem statement which concludes the proof.
\end{proof}

==> archive/wrong-proof.tex <==
\begin{claim}
For every strategy $S$,
$$\Rev^S(D^n) - \SP(D^n) < O(\rev(D))$$
\end{claim}
\begin{proof}
Let $Z = \sup_i X_i$ and observe that $\Rev^S(D^n) \leq E[Z]$ since in the worst case the auctioneer can force the highest bidder to pay his bid. Let $p$ denote the optimal reserve price, then
\begin{align*}
    \Rev^S(D^n) &- \SP(D^n) \leq E[Z] - E[\phi^+(Z)]\\
    &= E[Z \cdot \indicator{Z \leq p}] + E[Z \cdot \indicator{Z > p}] - E\bigg[\bigg(Z - \frac{1 - F(Z)}{f(Z)}\bigg)\cdot \indicator{Z > p}\bigg]\\
    &\leq p + E\bigg[\bigg(\frac{1 - F(Z)}{f(Z)}\bigg)\cdot \indicator{Z > p}\bigg]
\end{align*}
Because $F$ is MHR, we can bound $E\bigg[\bigg(\frac{1 - F(\sup X_i)}{f(\sup X_i)}\bigg)\bigg] \leq E\bigg[\bigg(\frac{1 - F(X_1)}{f(X_1)}\bigg)\bigg]$ since $\sup X_i \geq X_1$. For positive random variables, we have $E\bigg[\bigg(\frac{1 - F(X_1)}{f(X_1)}\bigg)\bigg] = E[X_1]$. Next we apply \Cref{lemma:extreme-value-mhr} on $X_1$ for $\varepsilon = 2^{-6}$ to bound $E[X_1]$.
\begin{align*}
    E[X_1] = E[X_1 \cdot \indicator{X_1 \leq 12B}] + E[X_1 \cdot \indicator{X > 12B}] \leq 12B + \frac{27}{2^3}B
\end{align*}
where $B$ is the anchoring point for $X_1$ which implies $B \leq \frac{2}{1-1/\sqrt{e}}\rev(D)$. Combining with the bound to the optimal reserve price,
\begin{align*}
    \Rev^S(D^n) - \SP(D^n) &\leq 22\rev(D) + \frac{2}{1-1/\sqrt{e}}(12 + 27/8)\rev(D)\\
    &< 101\rev(D)
\end{align*}
\end{proof}

\begin{theorem}
If bidders are i.i.d from a MHR distribution, then the second price auction with commitments is credible for $k = O(\rev(D))$.
\end{theorem}
\begin{proof}
Suppose for contradiction the auctioneer deviates and play strategy $S$ to get expected revenue $Rev^S(D^n)$. Let $Gain^S(D^n) := \Rev^S(D^n) - \SP(D^n)$ denote the extra profit of the auctioneer. Myerson optimal auctions imply that we must not sell an item if the highest bidder has negative virtual value. The reserve price $p$ is the value where $\phi(p) = 0$ and since $D$ is MHR, $\phi(x)$ is monotone increasing and we must sell as long as the highest bidder bids higher than $p$ and charge at least the reserve price $p$.

\begin{claim}
The optimal reserve $p$ is at most $\frac{44}{1-1/\sqrt{e}} \rev(D)$.
\end{claim}
\begin{proof}
Let $B$ denote the anchoring point as defined in \Cref{lemma:extreme-value-mhr} for a single draw from $D$. If we set a reserve price to $B/2$, we sell with probability at least $1-1/\sqrt{e}$; therefore, $\rev(D) \geq B/2 (1 - 1/\sqrt{e})$.

Assume for contradiction, the optimal reserve price $p > 2 B \log 1/\varepsilon$, for $\varepsilon = 1/2^{11}$,
\begin{align*}
    \rev(D) &= p Pr[X \geq p] \leq \int_{p}^\infty x Pr[X = x]dx\\
    &\leq 36 B \varepsilon \log 1/\varepsilon\\
    &< B/2 (1 - 1/\sqrt{e}) \Rightarrow\Leftarrow
\end{align*}
where the second inequality follows by the extreme value theorem for MHR distributions. In the third inequality, we reach a contradiction because setting a reserve of $B$ gives strictly higher revenue. This implies $p \leq 22B$ and because $B$ is a anchoring point, we have $B \leq \frac{2}{1 - 1/\sqrt{e}} \rev(D)$ which concludes the proof.
\end{proof}

\begin{claim}
For every strategy $S$,
$$\Rev^S(D^n) - \SP(D^n) < O(\rev(D))$$
\end{claim}
\begin{proof}
Let $Z = \sup_i X_i$ and observe that $\Rev^S(D^n) \leq E[Z]$ since in the worst case the auctioneer can force the highest bidder to pay his bid. Let $p$ denote the optimal reserve price, then
\begin{align*}
    \Rev^S(D^n) &- \SP(D^n) \leq E[Z] - E[\phi^+(Z)]\\
    &= E[Z \cdot \indicator{Z \leq p}] + E[Z \cdot \indicator{Z > p}] - E\bigg[\bigg(Z - \frac{1 - F(Z)}{f(Z)}\bigg)\cdot \indicator{Z > p}\bigg]\\
    &\leq p + E\bigg[\bigg(\frac{1 - F(Z)}{f(Z)}\bigg)\cdot \indicator{Z > p}\bigg]
\end{align*}
Because $F$ is MHR, we can bound $E\bigg[\bigg(\frac{1 - F(\sup X_i)}{f(\sup X_i)}\bigg)\bigg] \leq E\bigg[\bigg(\frac{1 - F(X_1)}{f(X_1)}\bigg)\bigg]$ since $\sup X_i \geq X_1$. For positive random variables, we have $E\bigg[\bigg(\frac{1 - F(X_1)}{f(X_1)}\bigg)\bigg] = E[X_1]$. Next we apply \Cref{lemma:extreme-value-mhr} on $X_1$ for $\varepsilon = 2^{-6}$ to bound $E[X_1]$.
\begin{align*}
    E[X_1] = E[X_1 \cdot \indicator{X_1 \leq 12B}] + E[X_1 \cdot \indicator{X > 12B}] \leq 12B + \frac{27}{2^3}B
\end{align*}
where $B$ is the anchoring point for $X_1$ which implies $B \leq \frac{2}{1-1/\sqrt{e}}\rev(D)$. Combining with the bound to the optimal reserve price,
\begin{align*}
    \Rev^S(D^n) - \SP(D^n) &\leq 22\rev(D) + \frac{2}{1-1/\sqrt{e}}(12 + 27/8)\rev(D)\\
    &< 101\rev(D)
\end{align*}
\end{proof}
\end{proof}

\begin{claim}
The optimal reserve $p$ is at most $\frac{44}{1-1/\sqrt{e}} \rev(D)$.
\end{claim}
\begin{proof}
Let $B$ denote the anchoring point as defined in \Cref{lemma:extreme-value-mhr} for a single draw from $D$. If we set a reserve price to $B/2$, we sell with probability at least $1-1/\sqrt{e}$; therefore, $\rev(D) \geq B/2 (1 - 1/\sqrt{e})$.

Assume for contradiction, the optimal reserve price $p > 2 B \log 1/\varepsilon$, for $\varepsilon = 1/2^{11}$,
\begin{align*}
    \rev(D) &= p Pr[X \geq p] \leq \int_{p}^\infty x Pr[X = x]dx\\
    &\leq 36 B \varepsilon \log 1/\varepsilon\\
    &< B/2 (1 - 1/\sqrt{e}) \Rightarrow\Leftarrow
\end{align*}
where the second inequality follows by the extreme value theorem for MHR distributions. In the third inequality, we reach a contradiction because setting a reserve of $B$ gives strictly higher revenue. This implies $p \leq 22B$ and because $B$ is a anchoring point, we have $B \leq \frac{2}{1 - 1/\sqrt{e}} \rev(D)$ which concludes the proof.
\end{proof}

==> discretization.tex <==
\begin{lemma}\label{lemma:discretization-exp-value}
If $D^\epsilon$ is the discretization of $D$, then $E_{X \leftarrow D}[X] - \epsilon \leq E_{X \leftarrow D^\epsilon}[X] \leq E_{X \leftarrow D}[X]$
\end{lemma}
\begin{proof}
For the lower bound,
\begin{align*}
    E_{X \leftarrow D^\epsilon}[X] &= \sum_{i = 0}^\infty i\epsilon Pr[X = i\epsilon]\\
    &= \sum_{i = 0}^\infty \int_{i\epsilon}^{(1+1)\epsilon} (i+1)\epsilon f(x) -\epsilon f(x) dx\\
    &\geq \sum_{i = 0}^\infty \int_{i\epsilon}^{(i+1)\epsilon} x f(x) dx - \epsilon\\
    &= E_{X \leftarrow D}[X] - \epsilon
\end{align*}
For the upper bound,
\begin{align*}
    E_{X \leftarrow D^\epsilon}[X] &= \sum_{i = 0}^\infty \int_{i\epsilon}^{(i+1)\epsilon} i\epsilon f(x)dx\\
    &\leq \sum_{i = 0}^\infty \int_{i\epsilon}^{(i+1)\epsilon} xf(x)dx\\
    &= E_{X \leftarrow D}[X]
\end{align*}
\end{proof}

\begin{lemma}
If $D^\epsilon$ is the discretization of $D$, then for all $v \in \mathbb R$, $Pr_{X \leftarrow D^\epsilon}[X \geq v] \leq Pr_{X \leftarrow D}[X \geq v]$.
\end{lemma}

==> extensive-form.tex <==

We use a extensive form game to specify the mechanism. A finite game in extensive form is a tuple $\Gamma = (\tree, \infset := (\infset_i)_{i \in N}, \action := \{A(I)\}_{I \in \infset}, \outcome := (\outcome_i)_{i \in N})$ where
\begin{itemize}
    \item $\tree = (V, v_0, T, D, p)$ is a finite tree with a set of nodes $V$, rooted on $v_0 \in V$, partitioned on a set of terminal nodes $T \subset V$ and decision nodes $D \subset V \setminus T$ with predecessor function $p : V \to D$.
    \item $\mathcal I$ is a partition of $D$ called an information partition where $\mathcal I_i$ is the information set of player $i$.
    \item $\action$ is the set of all actions partitioned on the set of actions available for each information set $I \in \infset$, $A(\mathcal I)$.
    \item $\outcome : T \to X$ is an outcome that map terminal nodes to a consequence on $X$.
\end{itemize}

\begin{definition}[Messaging Game \cite{akbarpour2018credible}]
A messaging game specify the model of communication between the auctioneer and the players and which information each player learns through the execution of the game:
\begin{itemize}
    \item Until the auctioneer decides to stop:
    \begin{itemize}
        \item The auctioneer selects an agent $i \in N$ and sends a message $m$ along with a set of acceptable replies $R$.
        \item Agent $i$ privately observes $(m, R)$ and chooses $r \in R$.
        \item The auctioneer privately observes $r$.
    \end{itemize}
    \item The auctioneer selects a consequence $x \in X$.
\end{itemize}
\end{definition}

We denote $\mathcal G$ as the set of all extensive form games and the messaging game as a tuple $(G, S)$ where $G \in \mathcal G$ and $S = (S_1, ..., S_n)$ is the strategy profile of $n$ players. We denote the auctioneer as the player zero with utility $u_0(S_0^G, S, \theta)$ where $S_0^G$ denotes the auctioneer's strategy implementing game $G$ and $\theta = (\theta_1, ..., \theta_n)$ is the private information of players. We assume $\theta$ is drawn independently from product distribution $D = \times_{i = 1}^n D_i$. We denote a strategy $S_0'^{G'}$ as a safe deviation from $G$ if no player can distinguish strategy $S_0'^{G'}$ from $S_0^G$.


==> malleableold.tex <==
\begin{definition}[Almost reasonable] We say that a commitment is \emph{loosely tied} to $(m_1,r_1),\ldots, (m_k, r_k)$ if the participant who sent $c$ explicitly computed a poly-time function of $c_1,\ldots, c_k$, which were explicitly tied to $(m_1,r_1),\ldots, (m_k,r_k)$. A deviation is \emph{almost reasonable with respect to $g$} for the auctioneer in the communication game is a strategy such that whenever the auctioneer reveals a commitment to $c$, with $c= \commit(m, r)$, then $m=g(m_1,\ldots, m_k)$ for some $(m_1,r_1),\ldots, (m_k,r_k)$ to which $c$ is loosely tied.
\end{definition}

To help get intuition for the definition above, observe that any reasonable deviation is also almost reasonable with respect to the identity function. If the commitment scheme is malleable, though, and it is possible to compute a poly-time function $g(\cdot,\ldots, \cdot)$ on commitments without being revealed, then a deviation which forwards a commitment to $g(b_1,\ldots, b_{n-1})$ to bidder $n$ (before the commitments are revealed), and then later reveals $g(b_1,\ldots, b_{n-1})$ is almost reasonable with respect to $g$. 

\begin{definition}[Strongly Computationally Credible] An auction is \emph{strongly computationally credible with respect to $g$} if, in expectation over $\vec{v} \leftarrow D$, and buyers being truthful, the auctioneer maximizes their expected revenue, over all deviations which are both safe and almost reasonable with respect to $g$, by executing the auction in earnest.

An auction is strongly $\varepsilon$-computationally credible with respect ot $g$ if executing the auction in earnest yields a $(1-\varepsilon)$-fraction of the expected revenue of any safe, almost reasonable with respect to $g$ deviation.
\end{definition}

Theorems~\ref{thm:malleable} and~\ref{thm:alphabounded} below show that, perhaps surprisingly, both assumptions of unbounded distributions and non-malleable commitment schemes are necessary for Theorem~\ref{thm:alphamhr} (whereas they were not necessary for Theorem~\ref{thm:mhr}, and appear to be just a technical artifact of our proof approach through Lemma~\ref{lem:all}). 

\begin{theorem}\label{thm:malleable} Let $g$ be any function such that $g(m_1,\ldots, m_k) \geq \max_{i \in [k]}\{m_i\}$. Then for all $\alpha < 1$, there exists a $D_0$ which is $\alpha$-strongly regular, such that for all $\varepsilon > 0$ and all $f(\cdot, \cdot)$, there exists a sufficiently large $n$ such that $\dra(f)$ is not strongly $(1-\alpha-\varepsilon)$-computationally credible with respect to $g$ for the instance $D:=\times_{i=1}^n D_0$.
\end{theorem}

In Theorem~\ref{thm:alphabounded} below, by the notation $D_0^T$, we mean the distribution $D_0$ \emph{truncated at $T$} (all probability mass above $T$ is moved to $T$. Formally, $\Pr_{v \leftarrow D_0}[v \geq x] = \Pr_{v \leftarrow D_0^T}[v \geq x]$ for all $x \leq T$, and $\Pr_{v \leftarrow D_0^T}[v \geq x] = 0$ for all $x > T$). 

\begin{theorem}\label{thm:alphabounded} For all $\alpha < 1$, there exists a distribution $D_0$ which is $\alpha$-strongly regular, such that for all $\varepsilon > 0$ and all $f(\cdot, \cdot)$ such that $f(n,D)$ depends on $\alpha, \varepsilon, r(D), n$ (but may depend arbitrarily on these values), there exists a sufficiently large $T$ and $n$ such that $\dra(f)$ is not $(1-\alpha-\varepsilon)$-credible for the instance $D:= \times_{i=1}^n D^T_0$.
\end{theorem}

The proofs of Theorems~\ref{thm:malleable} and~\ref{thm:alphabounded} will be nearly identical, and just wrap up differently at the end. Specifically, the $D_0$ for both theorems is the same, and the deviations are the same in spirit. First, we repeat the $D_0$ we use, which is the same from the proof of Theorem~\ref{thm:alphamhrneg}, repeated below for completeness:

\begin{minipage}{.5\linewidth}
$$F^\alpha(v) = \begin{cases}0 \quad & \text{, $v < 1$}\\
1 - \big(\frac 1 v\big)^{\frac 1 {1-\alpha}} \quad & \text{, $v \geq 1$} \end{cases}$$
\end{minipage}
\begin{minipage}{.5\linewidth}
$$f^\alpha(v) = \begin{cases} 0 \quad &\text{, $v < 1$}\\
\frac{1}{1-\alpha}\big(\frac 1 v\big)^{\frac {2-\alpha}{1-\alpha}} \quad &\text{, $v \geq 1$}\end{cases}$$
\end{minipage}

The hazard rate of $F^\alpha$ is $h^{F^\alpha}(v) = \frac{1}{(1-\alpha) v}$ for $v \geq 1$ and the virtual value function of $F^\alpha$ is $\varphi^{F^\alpha}(v) = v - \frac{1}{h^{F^\alpha}(v)} = \alpha v$, so $D_0$ is $\alpha$-strongly regular. 

Our proof will proceed as follows. First, we will quickly establish that $\rev(D) = \alpha \cdot \mathbb{E}_{\vec{v} \leftarrow D}[\max_i \{v_i\}]$. Then, we will design a deviation which achieves revenue arbitrarily close to $\mathbb{E}_{\vec{v} \leftarrow D}[\max_i \{v_i\}]$ for sufficiently large $n$. Finally, we will show that this deviation satisfies the properties of the two theorems (separately). 

\begin{claim} For any $n$, and $D:= D_0^n$, $\rev(D) = \alpha \cdot \cdot \mathbb{E}_{\vec{v} \leftarrow D}[\max_i \{v_i\}]$. 
\end{claim}
\begin{proof}
This could be verified by direct (but tedious) calculations. A simpler proof observes that $\rev(D)= \mathbb{E}[\max_i \{\varphi(v_i)\}]$ by Myerson's lemma. But because $\varphi(v_i):= \alpha v_i$, we immediately get that $\rev(D)= \mathbb{E}[\max_i \{\varphi(v_i)\}] = \alpha \cdot \mathbb{E}[\max_i \{\varphi(v_i)\}]$. 
\end{proof}

Now, consider the following deviation in $\dra(f)$. For any desired parameter $\delta$, we will argue that the following deviation gets revenue (not counting fines) at least $(1-\delta)\cdot \mathbb{E}[\max_i \{\varphi(v_i)\}]$, and also pays at most $\poly(1/\delta)$ fines. Importantly, \emph{the number of fines paid will depend only on $\delta$ and is independent of $n$} (it is not crucial that it is polynomial in $1/\delta$). 

Our deviation is as follows: for $i=0$ to $??$, let $x_\ell:= \delta \cdot (1+\delta)^\ell \cdot \rev(D)$. Upon receiving commitments to $b_1,\ldots, b_n$ from the bidders, the auctioneer will send to bidder $i$:
\begin{itemize}
\item A commitment to $x_\ell$, for all $\ell$.
\item A single additional commitment to $y^*_i$, where it is guaranteed that $b_i > y^*_i$ \emph{only if} $b_i > b_j$ for all $j \neq i$ (but perhaps $b_i > y^*_i$ for no $i$). Note that we defer to the last step of each proof exactly how to accomplish this. 
\end{itemize}

Next, the auctioneer will reveal commitments as follows:
\begin{itemize}
\item To all bidders $j \neq \arg\max_i \{b_i\}$, reveal all commitments. Note that this guarantees that bidder $j$ does not expect to win the item.
\item To bidder $i^* = \arg\max_i \{b_i\}$: 
\begin{itemize}
\item If $b_{i^*} < x_0$, reveal all commitments. 
\item If $b_{i^*} > x_{??}$, reveal all commitments except $y^*_{i^*}$.
\item If $b_{i^*} \in [x_\ell,x_{\ell_1})$, reveal commitments $x_0,\ldots, x_\ell$ and conceal the rest.
\end{itemize}
\end{itemize}



Now, we consider the safe, reasonable, deviation which sends to each bidder not only $\max_{j \neq i} \{b_j\}$, but also $c\cdot \max_{j \neq i} \{b_j\},\ldots, c^k \cdot \max_{j \neq i} \{b_j\}$ for appropriately chosen $c, k$ to be defined later. Below, let $X$ denote a random variable equal to the maximum of $n-1$ i.i.d. draws from $D_0$. 

\begin{observation}\label{obs:alphaexample} The expected payment made by bidder $i$ to the second-price auction, for all $i$, is $\mathbb{E}[X \cdot (1-F^\alpha(X))]$. Therefore, the expected revenue of the second-price auction is $n\cdot \mathbb{E}[X \cdot (1-F^\alpha(X))] = n \cdot \mathbb{E}[X^{-\frac{\alpha}{1-\alpha}}]$.
\end{observation}
\begin{proof}
The price set for bidder $i$ is distributed exactly according to $X$, and bidder $i$ pays this price whenever $v_i > X$, which happens with probability exactly $1-F^\alpha(X)$. The `Therefore,' portion of the claim follows by linearity of expectation.
\end{proof}

Consider instead the auction which commits to $\max_{j \neq i}\{b_j\}, c\cdot \max_{j \neq i} \{b_j\},\ldots, c^k \cdot \max_{j \neq i} \{b_j\}$ to bidder $i$ (for all $i$). If $b_i < \max_{j \neq i}\{b_j\}$, then reveal all commitments. Otherwise, reveal all commitments $< b_i$, and conceal all commitments $> b_i$. We now compute the revenue of this scheme \emph{excluding fines}.

\begin{claim}\label{claim:alphaexample} In the limit as $c \rightarrow 1$, and $k \rightarrow \infty$, the revenue (excluding fines) of the above safe, reasonable deviation approaches $\rev(D)/\alpha$. Therefore, for all $\varepsilon > 0$, there exists a sufficiently small $c > 1$ and large $k$ such that the revenue (excluding fines) of the above safe, reasonable deviation is at least $\rev(D)/(\alpha + \varepsilon)$.
\end{claim}
\begin{proof}
Considering the limit as $k \rightarrow \infty$, the payment made by bidder $i$ in this safe, reasonable deviation is $0$ if $v_i < \max_{j \neq i} \{v_j\}$, and equal to $c^\ell\max_{j \neq i} \{v_j\}$ whenever $v_i \in [c^\ell\max_{j \neq i} \{v_j\}, c^{\ell+1} \max_{j \neq i} \{v_j\})$. For ease of notation and letting $X:= \max_{j \neq i} \{v_j\}$, we find that this occurs with probability exactly:

\begin{align*}
F^\alpha(c^{\ell+1}X) - F^\alpha(c^\ell X) &= 1-(c^{\ell+1}X)^{\frac{-1}{1-\alpha}} - (1- (c^{\ell}X)^{\frac{-1}{1-\alpha}}) \\
&= X^{\frac{-1}{1-\alpha}} c^{\frac{-\ell}{1-\alpha}} \cdot \left(1 - c^{\frac{-1}{1-\alpha}}\right)\\
\end{align*}

Therefore, the revenue of this scheme as $k \rightarrow \infty$, ignoring fines, is exactly (where we have multiplied by $n$ to count all buyers, and the expectation is taken over the buyers $\neq i$):

\begin{align*}
n \cdot \mathbb{E}\left[\sum_{\ell = 0}^\infty (Xc^\ell) \cdot X^{\frac{-1}{1-\alpha}} c^{\frac{-\ell}{1-\alpha}} \cdot \left(1 - c^{\frac{-1}{1-\alpha}}\right)\right] &= n \cdot \left(\sum_{\ell=0}^\infty c^{\frac{-\ell \alpha}{1-\alpha}}\right) \cdot \left(1-c^{\frac{-1}{1-\alpha}}\right)\cdot \mathbb{E}[X^{\frac{-\alpha}{1-\alpha}}]\\
&=n \cdot \mathbb{E}[X^{\frac{-\alpha}{1-\alpha}}] \cdot \frac{1-c^{\frac{-1}{1-\alpha}}}{1-c^{\frac{-\alpha}{1-\alpha}}}
\end{align*}

Now, we want to take the limit as $c \rightarrow 1$. Observe that the fraction is $0/0$ in the limit, so we may use L'Hopitals rule, which gives that the limit as $c \rightarrow 1$ is: $\frac{c^{\frac{-1}{1-\alpha}-1}/(1-\alpha)}{\alpha \cdot c^{\frac{-\alpha}{1-\alpha}-1}/(1-\alpha)}$. As $c \rightarrow 1$, this is now $1/\alpha$.

Finally, observe that this means that the revenue is $n \cdot \mathbb{E}[X^{\frac{-\alpha}{1-\alpha}}]/\alpha$, exactly the revenue of the second price auction (by Observation~\ref{obs:alphaexample}) divided by $\alpha$. The `Therefore,' portion of the claim follows by taking sufficiently large $k$ and small $c> 1$.
\end{proof}

Now, we are ready to wrap up the proof. We just need to account for fines. Observe, first, that Claim~\ref{claim:alphaexample} is \emph{independent of $n$}. That is, for any $\varepsilon$, we can pick a $c,k$, such that the revenue (ignoring fines) of the safe, reasonable deviation is at least $\rev(D)/(\alpha+\varepsilon)$ \emph{for all $n$}. So say that we would like an instance where this safe, reasonable deviation gets revenue at least $\rev(D)/(\alpha+\varepsilon')$. We will first set $\varepsilon = 2\varepsilon'$, and see what choice of $c, k$ we need for this guarantee. Next, we see how large $f(k+1,D_0)$ is, and observe that this safe, reasonable deviation will never pay more than $k\cdot f(k+1,D_0)$ in fines (because it only makes $k$ commitments which are ever concealed). Therefore, our total revenue on any instance would be:

$$\rev(D)/(\alpha + 2\varepsilon') - k \cdot f(k+1,D_0).$$

But beacuse $D_0$ is unbounded, there is a sufficiently large $n$ such that $k \cdot f(k+1,D_0) < \rev(D)\cdot \left(\frac{1}{\alpha+\varepsilon '}-\frac{1}{\alpha + 2\varepsilon'}\right)$ (just because as $n \rightarrow \infty, \rev(D) \rightarrow \infty$). So for this sufficiently large $n$, the fines are small enough that even if they are paid with probability one, its impact on the revenue is negligible. This completes the proof.
\end{proof}

Finally, we show that Theorem~\ref{thm:malleable} is tight. In the proof of Theorem~\ref{thm:malleable2} below, note that Lemma~\ref{lem:onebig} and Corollary~\ref{cor:alphanonebig} only require that $\beta_i$ is a function of $\vec{b}_{-i}$, and not that it takes a particular (non-malleable) form.

\begin{theorem}\label{thm:malleable2}
Let $f(n, D_i) := r(D_i)$. Then when all $D_i$ are $\alpha$-strongly regular (bounded or unbounded), $DRA(f)$ is optimal, strategyproof, and $(1-\alpha)$-credible.
\end{theorem}
\begin{proof}
Let $k_i = r(D_i)$. Recall $X_i(\vec v)$ is the indicator variable for the event where the item is allocated to buyer $i$ and $k_i \leq v_i < \beta_i$. Also observe that $\bar \phi_i(v_i) = \phi_i(v_i)$ since $D_i$ is regular. If $X_i(\vec v) = 1$, then $v_i \geq k_i \geq r_i$ and by definition $\phi_i(v_i) \cdot X_i(\vec v) \geq 0$. We first combine Lemma~\ref{lem:onebig} and Corollary~\ref{cor:alphanonebig}:
\begin{align*}
    \mathbb{E}_{\vec{v} \leftarrow D}[R(\vec{v})] &=\mathbb{E}_{\vec{v} \leftarrow D}[R(\vec{v}) \cdot I(\exists\ i, v_i > \beta_i)] + \mathbb{E}_{\vec{v} \leftarrow D}[R(\vec{v}) \cdot I(\forall\ i, v_i < \beta_i)]\\
    &\leq\mathbb{E}_{\vec{v} \leftarrow D}[\max_i\{\varphi_i(v_i)\} \cdot I(\exists\ i, v_i > \beta_i)] + \sum_{i=1}^n\mathbb{E}_{\vec{v} \leftarrow D}[(\varphi_i(v_i)/\alpha + r(D_i) - k_i) \cdot X_i(\vec v)]\\
    &\leq \mathbb{E}_{\vec{v} \leftarrow D}[\max_i\{\varphi_i(v_i)\}] + \sum_{i = 1}^n \mathbb{E}_{\vec{v} \leftarrow D}[\varphi_i(v_i)/\alpha\cdot X_i(\vec v)] - \mathbb{E}_{\vec{v} \leftarrow D}[\max_i\{\varphi_i(v_i)\} \cdot I(\forall i, v_i < \beta_i)]\\
    &\leq \rev(D) + \sum_{i = 1}^n\mathbb{E}_{\vec{v} \leftarrow D}[\varphi_i(v_i)/\alpha \cdot X_i(\vec v)] - \sum_{i=1}^n \mathbb{E}_{\vec{v} \leftarrow D}[\varphi_i(v_i) \cdot X_i(\vec v) \cdot I(\forall i, v_i < \beta_i)]\\
    &\leq \rev(D) + \sum_{i = 1}^n\mathbb{E}_{\vec{v} \leftarrow D}[(1-\alpha)\varphi_i(v_i)/\alpha \cdot X_i(\vec v)]\\
    &\leq \rev(D) + \frac{1-\alpha}{\alpha} \rev(D)\\
    &= \frac{1}{\alpha} \rev(D)
\end{align*}
\end{proof}
The first line is just linearity of expectation. The second line combines Lemma~\ref{lem:onebig} and Corollary~\ref{cor:alphanonebig}. The third line is again by linearity of expectation and the fact $k_i = r(D_i)$. The fourth line uses the fact that $\mathbb{E}_{\vec{v} \leftarrow D}[\max_i\{\varphi_i(v_i)\}]$ is the revenue of Myerson's optimal auction and $\max(\varphi_i(v_i)) \geq \sum_{i = 1}^n \varphi_i(v_i)\cdot X_i(\vec v)$ since the indicator random variable $X_i(\vec v) = 1$ for at most one bidder. The fifth line is just the fact $X_i(\vec v) = 1$ implies $\forall i, v_i < \beta_i$ and by linearity of expectation. In the sixth line, we observe that the second term is at most the revenue of the second price auction.


==> setup.tex <==
\makeatletter
\def\renewtheorem#1{%
  \expandafter\let\csname#1\endcsname\relax
  \expandafter\let\csname c@#1\endcsname\relax
  \gdef\renewtheorem@envname{#1}
  \renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{  
\def\renewtheorem@caption{#1}
\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

\makeatletter
% \saveequation{<ID>}{<equation>}
\newcommand\saveequation[2]{%
  \@namedef{equation@#1}{#2}%
}

% \useequation{<ID>}
\newcommand\useequation[1]{%
  \@nameuse{equation@#1}%
}
\makeatother

\usepackage{color}
\usepackage{amsmath,hyperref}
\usepackage{amsthm}
\usepackage{filecontents}
\usepackage[utf8]{inputenc}
\usepackage{booktabs} % For formal tables
\usepackage{algorithmic}
\usepackage[ruled]{algorithm2e}
\usepackage[normalem]{ulem}
\usepackage{aliascnt}
\usepackage{cleveref}
\usepackage{amsfonts}
\usepackage[normalem]{ulem}

\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}
\IncMargin{-\parindent}
\newcommand{\mattnote}[1]{\textcolor{blue}{#1}}
\newcommand{\mathnote}[1]{{\color{red}#1}}
\Crefname{algocf}{Algorithm}{Algorithms}
\Crefname{lemma}{Lemma}{Lemmas}
\Crefname{corollary}{Corollary}{corollaries}
\Crefname{claim}{Claim}{Claims}
\renewtheorem{proposition}{Proposition}[section]
\renewtheorem{corollary}{Corollary}[section]
\renewtheorem{lemma}{Lemma}[section]
\renewtheorem{definition}{Definition}[section]
\renewtheorem{example}{Example}[section]
\renewtheorem{theorem}{Theorem}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{construction}{Construction}[section]
\newtheorem{assumption}{Assumption}[section]


\newcommand{\poly}{\text{poly}}
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\renewcommand{\max}{\text{max}}
\newcommand{\commit}{\ensuremath{\textsf{Commit}}}
\newcommand{\fee}{k}
\newcommand{\rev}{\ensuremath{\textsf{Rev}}}
\newcommand{\slog}{\ln^*}
\newcommand{\Rev}{Rev}
\newcommand{\SP}{\Rev^{SP}}
\newcommand{\indicator}[1]{\mathbb I[#1]}
\newcommand{\protocol}{\mathcal M}
\newcommand{\HIDE}{\text{HIDE}}
\newcommand{\HONEST}{\text{HONEST}}
\newcommand{\tree}{\Gamma}
\newcommand{\infset}{\mathcal I}
\newcommand{\action}{\mathcal A}
\newcommand{\outcome}{O}
\newcommand{\exec}{\mathcal S}
\newcommand{\sspc}{\mathcal S^{SPC}}
\newcommand{\funcommit}{\mathcal F_{COM}}
\newcommand{\strawman}{\ensuremath{\mathsf{Strawman}}}
\newcommand{\dra}{\ensuremath{\mathsf{DRA}}}
